Robust Reinforcement Learning Under Minimax Regret for Green Security

Green security domains feature defenders who plan patrols in the face of uncertainty about the adversarial behavior of poachers, illegal loggers, and illegal fishers. Importantly, the deterrence effect of patrols on adversaries' future behavior makes patrol planning a sequential decision-making problem. Therefore, we focus on robust sequential patrol planning for green security following the minimax regret criterion, which has not been considered in the literature. We formulate the problem as a game between the defender and nature who controls the parameter values of the adversarial behavior and design an algorithm MIRROR to find a robust policy. MIRROR uses two reinforcement learning-based oracles and solves a restricted game considering limited defender strategies and parameter values. We evaluate MIRROR on real-world poaching data.

==> deterrence.tex <==
\section{Deterrence Analysis}
\label{sec:deterrence}

Poachers are strategic and wish to place snares in places that are less likely to be detected and removed by rangers. However, the question of \emph{how} poachers respond to ranger patrols remains an open question. We analyze real-world poaching data from two national parks in Uganda to learn poacher behavior, which serves as the foundation to our model. 


Our analysis of poacher behavior, which shows deterrence, provides our adversarial model for green security domains. 


We consider robust planning in the poaching domain where the poacher is a reactive adversary. The likelihood that poaching occurs at a given target is governed by (1)~the rangers' past patrol effort at that target (deterrence), (2)~the rangers' past patrol effort at neighboring targets (displacement), and (3)~the base attractiveness of the target. Factors (1) and (2) are ones we as the defender can control; (3) is determined by Nature and the exact values are unknown, but are drawn from a known interval.


We consider the domain of wildlife protection, in which rangers conduct patrols to confiscate snares set up by poachers to trap animals. We consider a park discretized into $1 \times 1$~km cells (targets). At each timestep poachers can choose whether to place a snare in each of the targets. Rangers can patrol targets up to their total allocation of effort for the timestep. Their probability of detecting the snare, assuming that one is placed, is determined by a piecewise-linear function dependent on effort expended. 

Past work focused on patrol planning by optimizing patrol routes assuming a stochastic adversary and determining one-shot planning in response. However, a stochastic adversary is not realistic, given that we would expect the adversary to change their behavior depending on the rangers' actions. 
Some papers \citep{fang2015security} consider a game-theoretic adversary based on an SUQR model. However, this model is not justified with real-world data. 

We therefore consider a sequential decision-making problem, in which our actions impact the future. We learn the poachers' behavioral model from real-world data. Specifically, we show both a \textit{deterrence} effect, where poaching probability decreases with past patrol effort, and a \textit{displacement} effect, where increased patrolling at one target increases poaching probability at neighboring targets. The displacement effect suggests a hotspot pattern to poaching: various regions are attractive to poachers, and if we patrol heavily in one region, poachers will simply move to a different target within that hotspot. 

In a traditional Stackelberg game, the defender (leader) plays first. The adversary then best responds after observing the defender strategy to act accordingly. Our domain instead exhibits \textit{delayed feedback} in which the adversary is not able to observe the defender's strategy until after the turn ends. Thus, we have a reactive adversary who changes his behavior in response to the defender's past action. In this way, we have a simultaneous-move game with delayed feedback to the adversary. 

Note that in this model, the attacker is not a game-theoretic adversary in a classical sense. Instead, the attacker is a reactive adversary that can be modeled as part of the environment, with a response pattern that can be specified in advance. 

Unfortunately, the available data from ranger patrols are incomplete, as they are unable to observe every poacher attack. So although we are able to learn an approximate model of poacher behavior, we do not have a perfect certainty in the parameters, nor do we have a reliable estimate of the distribution over the uncertainty intervals. 



==> figures/plot_ablation.tex <==
\begin{tikzpicture}
\pgfplotsset{
  %scale only axis,
  width=.8\linewidth,
  height=0.42\linewidth,
  xtick pos=left,
  ytick pos=left,
  tick label style={font=\scriptsize},
  ymajorgrids=true,
}

% ----------------------------------------------------------
% ablation
\begin{axis}[
%   width=0.34\linewidth,
%   at={(.66\linewidth, 0\linewidth)},
  table/col sep=comma,
  ybar,
%   ybar=1,
%   ybar interval=.8,
  bar width=.2cm,
  % x tick label style={rotate=90,anchor=east}
  symbolic x coords={all, no wake-sleep, no perturb, neither},
  xtick={data},
  xticklabels={WS+P, No WS, No P, Neither},
  xlabel={\footnotesize{Ablation study}}, 
%   ylabel style={align=center},
%   ylabel={\footnotesize{Max regret}},
%   ylabel shift = -2pt,
%   title={Ablation},
  legend style={
    at={(1.05,1.26)},
    legend columns=3,
    font=\small,draw=none,fill=none},
%   xmin=0,xmax=11,
  ymin=0.1, %ymax=10,
% enlargelimits=true,
  enlarge x limits={0.2},
  error bars/y dir=both, % turn on error bars
  error bars/y explicit,  % say that error value is given explicitly
  error bars/error bar style={color=black, thick},
]

% bar plots
\addplot+[cyan!70!white, draw=black, thick, area legend,
postaction={pattern=north east lines,}
] table [x=setting, y=do]{data/ablation.csv};
%, y error=do_stderr]

\end{axis}

% \begin{axis}[
%   at={(0\linewidth, .22\linewidth)},
%   table/col sep=comma,
%   ybar,
% %   ybar=1,
% %   ybar interval=.8,
%   bar width=.2cm,
%   % x tick label style={rotate=90,anchor=east}
%   symbolic x coords={all params, no wake/sleep, no perturb},
%   xtick={data},
%   xticklabels={All, No wake--sleep, No perturb},
% %   xlabel={\footnotesize{(a) Budget~$B$}}, 
% %   ylabel style={align=center},
%   ylabel={\footnotesize{Max regret}},
%   ylabel shift = -2pt,
% %   title={\textbf{(a) Vary Budget}},
%   legend style={
%     at={(1.05,1.26)},
%     legend columns=3,
%     font=\small,draw=none,fill=none},
% %   xmin=0,xmax=11,
%   ymin=0.1, %ymax=10,
% % enlargelimits=true,
%   enlarge x limits={0.2},
% ]

% % bar plots
% \addplot+[cyan!70!white, draw=black, thick, area legend,
% postaction={
%     pattern=north east lines,
%     % pattern color=white,
% }
% ] table [x=setting, y=do] {data/ablation.csv}; %\addlegendentry{MIRROR};
% % \addplot+[red!70!white, draw=black, thick, area legend,
% % postaction={
% %     pattern=dots,
% %     % pattern color=white,
% % }
% % ] table [x=setting, y=middle] {data/ablation.csv}; \addlegendentry{middle};
% % \addplot+[yellow!90!white, draw=black, thick, area legend,
% % postaction={pattern=horizontal lines,}
% % ] table [x=setting, y=random] {data/ablation.csv}; \addlegendentry{random};
% \end{axis}

\end{tikzpicture}

